TSViz: Demystification of Deep Learning Models for Time-Series Analysis

This paper presents a novel framework for demystification of convolutional deep learning models for time-series analysis. This is a step towards making informed/explainable decisions in the domain of time-series, powered by deep learning. There have been numerous efforts to increase the interpretability of image-centric deep neural network models, where the learned features are more intuitive to visualize. Visualization in time-series domain is much more complicated as there is no direct interpretation of the filters and inputs as compared to the image modality. In addition, little or no concentration has been devoted for the development of such tools in the domain of time-series in the past. TSViz provides possibilities to explore and analyze a network from different dimensions at different levels of abstraction which includes identification of parts of the input that were responsible for a prediction (including per filter saliency), importance of different filters present in the network for a particular prediction, notion of diversity present in the network through filter clustering, understanding of the main sources of variation learnt by the network through inverse optimization, and analysis of the network's robustness against adversarial noise. As a sanity check for the computed influence values, we demonstrate results regarding pruning of neural networks based on the computed influence information. These representations allow to understand the network features so that the acceptability of deep networks for time-series data can be enhanced. This is extremely important in domains like finance, industry 4.0, self-driving cars, health-care, counter-terrorism etc., where reasons for reaching a particular prediction are equally important as the prediction itself. We assess the proposed framework for interpretability with a set of desirable properties essential for any method.

==> AnalysisAndDiscussion.tex <==
\section{Analysis and Discussion} \label{sec:analysisAndDiscussion}
This section is explicitly focused on providing detailed insights regarding different dimensions from which a network can be explored.  
In particular, the TSViz toolbox provides possibility to explore and analyze the given network at four different levels of abstraction. 
\begin{figure}[b]
    \centering
    \includegraphics[width=0.7\columnwidth]{Images/1_Main.png}
    \caption{Abstract representation of the network (First Level)} 
    \label{fig:1_overview}
\end{figure}

\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.70\textwidth]{Images/3-sorted-crop.png}
    \caption{Filters sorted according to their importance (Second level)} 
    \label{fig:3_detailed_view_sorted}
\end{figure*}

\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.70\textwidth]{Images/4-sorted-crop.png}
    \caption{Filters sorted according to their importance in descending order (Second level)} 
    \label{fig:4_detailed_view_reverse_sorted}
\end{figure*}

The first level provides the most abstract representation of the complete network. This provides the user with the opportunity to get himself acquainted with the network in question by providing a simplistic view of the network architecture highlighting the number of convolutional, max-pooling and dense layers present in the network along with the original input signal in question. The user can switch to the detailed view through the defined shortcut keys. The visualization is created in 3D so the user can change his perspective, but the frontal view is the most appropriate for understanding due to its simplicity. Figure~\ref{fig:1_overview} provides an overview of the complete network architecture both visually and in textual form. 

The second level extends the network architecture overview to display the original filters instead of dummy-blocks. This view is designed to get an overall idea regarding the learning of the network. We leverage conventional line plots which is one of the best known techniques for this purpose. Figure~\ref{fig:3_detailed_view_sorted} and Figure~\ref{fig:4_detailed_view_reverse_sorted} provides an unfolded view of the network. The plots in a particular layer are stacked in the depth dimension which the user can scroll through using the mouse-wheel to get an idea about the different filters present in a particular layer. As the user scrolls through the different filters within a layer, the input automatically adapts to demonstrate the influence of the input on the particular layer in question. The color strength of the red bar (Figure~\ref{fig:11_annotated_image}) on top of each filter indicates its impact on the final output i.e. the filter's importance. The filters with higher importance pops out of the stack with the height being proportional to its importance. The user has the possibility to sort the filters in ascending or descending order w.r.t. their importance as presented in Figure~\ref{fig:3_detailed_view_sorted} and Figure~\ref{fig:4_detailed_view_reverse_sorted} respectively.

The third level focuses on a particular layer instead of the whole network. This view displays all the filters in a particular layer stacked on a 2D grid in order to be able to inspect the layer in detail. This view again supports sorting w.r.t. to the filter importance within a particular layer. Just like the first view, the third view retains the input and output plots in order to make sure that the user is equipped with all the important information for analysis. Figure~\ref{fig:filters_and_clusters}(a) provides a depiction of the third level.

The fourth level further enhances the information from the third level by additionally visualizing the information regarding the filter clusters. Filters with similar activating patterns belongs to the same cluster. The clusters are represented via a colored bar on the left side of the plot. Filters belonging to the same cluster has the same color bar. Figure~\ref{fig:filters_and_clusters}(b) provides a depiction of the fourth level, where it can be clearly seen that all the filters in first cluster have no activity for that particular input. These filters amounts to a large fraction of the total filters present in the layer. Similarly, other clusters discovered by the system demonstrates consistency in the trend disregarding the scale.

\begin{figure*}
\centering
\subfloat[]{\includegraphics[width=0.80\columnwidth]{Images/5-crop.png}
\label{fig:a}}
\hfil
\subfloat[]{\includegraphics[width=0.80\columnwidth]{Images/6-crop.png}
\label{fig:b}}
\caption{Filters stacked on 2D grid (Third level - left) along with information regarding the filter cluster (Fourth level - right). All the filters are sorted w.r.t. their importance. }
\label{fig:filters_and_clusters}
\end{figure*}

Ability to take a look at the items within the receptive field of a particular neuron which were responsible to produce that particular value is essential for in-depth understanding of the network. Therefore, the visualization framework is equipped with Recursive highlightion feature which highlights the points which are actually responsible for the activation value obtained at that particular point. Adding lines to demonstrate the influence was problematic as the scene becomes cluttered with useless items. In order to highlight the points which are responsible, we add a light emission property to these points along with increased diameter making them stand out from the rest of the values. This feature enables the user to understand the flow of information. The feature is highlighted in Figure~\ref{fig:recursive_and_influence}. It is important to note that instead of visualizing all the values within the receptive field of the neuron, we only visualize the values which were actually responsible to produce the current activation, therefore, we only trace the maximum values through the max-pooling layers as the suppressed values have no impact onto the obtained activation.

\begin{figure*}[!h]
\centering
\subfloat[]{\includegraphics[width=0.7\columnwidth]{Images/7_Recursive_highlightion.png}
\label{fig:a}}
\hfil
\subfloat[]{\includegraphics[width=0.7\columnwidth]{Images/8_Input_influence_trace_2.png}
\label{fig:b}}
\caption{Recursive highlightion (left) and influence tracing of the input (right)}
\label{fig:recursive_and_influence}
\end{figure*}



Since a network can be comprised of a large number of filters, the system is equipped with a percentile constraint where the user can specify the importance percentile so that only the filters which exceed that importance percentile are visualized within each layer to allow the user to focus on the more important details. Figure~\ref{fig:9_percentile_filter} provides a glimpse of the percentile filter in action. In this case, the network is same as the one presented in Figure~\ref{fig:3_detailed_view_sorted} and Figure~\ref{fig:4_detailed_view_reverse_sorted} but only visualizes the filters which were most important due to the percentile filter being set to the 90\textsuperscript{th} percentile.

\begin{figure*}[!h]
    \centering
    \includegraphics[width=0.78\textwidth]{Images/9_percentile-crop1.png}
\caption{Application of the percentile filter on the detailed view (Second level)} 
    \label{fig:9_percentile_filter}
\end{figure*}

The visualization enabled a detailed inspection of the network which highlighted many different aspects of the network's learning.

\begin{itemize}
\item Most of the filters in the network were useless i.e. they contributed nothing to the final prediction for that particular input. These filters changed as the stimulus to the network changed indicating that some filters were specialized in a particular input.
\item Many of the filters had very similar activating patterns in the network which were assigned to the same filter cluster. This highlighted the aspect of lack of diversity in the trained network.
\item Despite of the improvement in performance with the addition of the first-order derivative of the original signal, most of the filters strongly attended to the original signal as compared to the first-order derivative.
\end{itemize}




==> Implementation.tex <==
\section{Implementation} \label{sec:implementation}

We used Keras with TensorFlow backend~\cite{chollet2015keras,tensorflow2015-whitepaper} developed specifically for deep learning. TensorFlow is an automatic differentiation package which enables automatic computation of the gradients. We leveraged this capability to compute the influences as described in section ~\ref{sec:approach}. We opt for two different use cases common in time series regime: Time series classification and time series regression.

For the classification use case, we created a dummy time-series anomaly detection dataset for binary classification. The dataset is comprised of 60000 sequences of 50 time-steps each where each time-step contains values for pressure, temperature and torque. We randomly introduce point anomalies in the dataset and mark the sequences containing such point anomalies as anomalous. We never introduced any anomalies in the pressure signal. The dataset is split into 50000 train sequences, 5000 validation, and 10000 test sequences. 
The network is comprised of three convolutional layers comprising of 16, 32 and 64 filters respectively followed by a single dense layer. The network is trained using binary cross-entropy loss. %

For the regression use case, we trained a network on Internet Traffic Dataset~\cite{cortez2012multi} for time series forecasting (we only used the B5M dataset out of the six available variants). The network operates on the input size of 50 time-stamps and is comprised of three convolution, two max-pooling and one dense layer. The network is trained using Adam optimizer with a learning rate of 0.001 for 5000 epochs using a batch size of 5 and mean squared error as the loss function. This network was able to achieve state-of-the-art forecasting results on the aforementioned dataset. The network takes in a bi-channel input where the first channel corresponds to the original input signal while the second channel is comprised of the first-order derivative of the original signal.

The front-end for the visualization toolbox is developed using Unity Game Engine~\cite{unityGameEngine} which communicates with the back-end exposed as a RESTful API. This decouples the model from the visualization aspect. 
Even though the focus of our work was on time series data, the system is generally applicable to any deep learning model as the it is only dependent on the effective computation of the gradients.

For pruning tests, we additionally included time-series regression datasets from UCL machine learning repository\footnote{https://archive.ics.uci.edu/ml/datasets}. The first dataset was regarding prediction of air quality called as the Air Quality Dataset\footnote{https://archive.ics.uci.edu/ml/datasets/Air+quality}. The dataset is comprised of 9358 instances divided into 70\% and 30\% ratio for training and test set respectively.
The next dataset we evaluated was PM2.5 Prediction Dataset\footnote{https://archive.ics.uci.edu/ml/datasets/Beijing+PM2.5+Data} for the US Embassy in Beijing. This dataset is comprised of 43824 instances. The details for all three datasets are presented in Table~\ref{tab:datasets}.

\begin{table}
\scriptsize
\renewcommand{\arraystretch}{1.0}
\caption{Datasets}
\label{tab:datasets}
\centering
\begin{tabular}{|c|c|c|}
\hline
\bfseries Dataset Name & \bfseries Data Instances & \bfseries Train/Test Split \\
\hline\hline

Internet Traffic Dataset & 18,000 & 78/28 \% \\
Air Quality Dataset & 9,358 & 70/30 \% \\
PM2.5 Prediction Dataset & 43,824 & - \\

\hline


\end{tabular}
\end{table}


==> tsviz-tool-old.tex <==
\section{TSViz - The toolbox} \label{sec:toolbox}
This section is explicitly focused on providing detailed insights regarding different dimensions from which a network can be explored using the tool.  
In particular, the TSViz toolbox provides possibility to explore and analyze the given network at four different levels of abstraction. 
\begin{figure}[b]
    \centering
    \includegraphics[width=0.7\columnwidth]{Images/1_Main.png}
    \caption{Abstract representation of the network (First Level)} 
    \label{fig:1_overview}
\end{figure}

\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.70\textwidth]{Images/3-sorted-crop.png}
    \caption{Filters sorted according to their importance (Second level)} 
    \label{fig:3_detailed_view_sorted}
\end{figure*}

\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.70\textwidth]{Images/4-sorted-crop.png}
    \caption{Filters sorted according to their importance in descending order (Second level)} 
    \label{fig:4_detailed_view_reverse_sorted}
\end{figure*}

The first level provides the most abstract representation of the complete network. This provides the user with the opportunity to get himself acquainted with the network in question by providing a simplistic view of the network architecture highlighting the number of convolutional, max-pooling and dense layers present in the network along with the original input signal in question. The user can switch to the detailed view through the defined shortcut keys. The visualization is created in 3D so the user can change his perspective, but the frontal view is the most appropriate for understanding due to its simplicity. Fig.~\ref{fig:1_overview} provides an overview of the complete network architecture both visually and in textual form. 

The second level extends the network architecture overview to display the original filters instead of dummy-blocks. This view is designed to get an overall idea regarding the learning of the network. We leverage conventional line plots which is one of the best known techniques for this purpose. Fig.~\ref{fig:3_detailed_view_sorted} and Fig.~\ref{fig:4_detailed_view_reverse_sorted} provides an unfolded view of the network. The plots in a particular layer are stacked in the depth dimension which the user can scroll through using the mouse-wheel to get an idea about the different filters present in a particular layer. As the user scrolls through the different filters within a layer, the input automatically adapts to demonstrate the influence of the input on the particular layer in question. The color strength of the red bar (Fig.~\ref{fig:conv2_imp}) on top of each filter indicates its impact on the final output i.e. the filter's importance. The filters with higher importance pops out of the stack with the height being proportional to its importance. The user has the possibility to sort the filters in ascending or descending order w.r.t. their importance as presented in Fig.~\ref{fig:3_detailed_view_sorted} and Fig.~\ref{fig:4_detailed_view_reverse_sorted} respectively.

The third level focuses on a particular layer instead of the whole network. This view displays all the filters in a particular layer stacked on a 2D grid in order to be able to inspect the layer in detail. This view again supports sorting w.r.t. to the filter importance within a particular layer. Just like the first view, the third view retains the input and output plots in order to make sure that the user is equipped with all the important information for analysis. Fig.~\ref{fig:filters_and_clusters}(a) provides a depiction of the third level.

The fourth level further enhances the information from the third level by additionally visualizing the information regarding the filter clusters. Filters with similar activating patterns belongs to the same cluster. The clusters are represented via a colored bar on the left side of the plot. Filters belonging to the same cluster has the same color bar. Fig.~\ref{fig:filters_and_clusters}(b) provides a depiction of the fourth level, where it can be clearly seen that all the filters in first cluster have no activity for that particular input. These filters amounts to a large fraction of the total filters present in the layer. Similarly, other clusters discovered by the system demonstrates consistency in the trend disregarding the scale.

\begin{figure*}
\centering
\subfloat[]{\includegraphics[width=0.80\columnwidth]{Images/5-crop.png}
\label{fig:a}}
\hfil
\subfloat[]{\includegraphics[width=0.80\columnwidth]{Images/6-crop.png}
\label{fig:b}}
\caption{Filters stacked on 2D grid (Third level - left) along with information regarding the filter cluster (Fourth level - right). All the filters are sorted w.r.t. their importance. }
\label{fig:filters_and_clusters}
\end{figure*}

Ability to take a look at the items within the receptive field of a particular neuron which were responsible to produce that particular value is essential for in-depth understanding of the network. Therefore, the visualization framework is equipped with Recursive highlightion feature which highlights the points which are actually responsible for the activation value obtained at that particular point. Adding lines to demonstrate the influence was problematic as the scene becomes cluttered with useless items. In order to highlight the points which are responsible, we add a light emission property to these points along with increased diameter making them stand out from the rest of the values. This feature enables the user to understand the flow of information. The feature is highlighted in Fig.~\ref{fig:recursive_and_influence}. It is important to note that instead of visualizing all the values within the receptive field of the neuron, we only visualize the values which were actually responsible to produce the current activation, therefore, we only trace the maximum values through the max-pooling layers as the suppressed values have no impact onto the obtained activation.

\begin{figure*}[!h]
\centering
\subfloat[]{\includegraphics[width=0.7\columnwidth]{Images/7_Recursive_highlightion.png}
\label{fig:a}}
\hfil
\subfloat[]{\includegraphics[width=0.7\columnwidth]{Images/8_Input_influence_trace_2.png}
\label{fig:b}}
\caption{Recursive highlightion (left) and influence tracing of the input (right)}
\label{fig:recursive_and_influence}
\end{figure*}



Since a network can be comprised of a large number of filters, the system is equipped with a percentile constraint where the user can specify the importance percentile so that only the filters which exceed that importance percentile are visualized within each layer to allow the user to focus on the more important details. Fig.~\ref{fig:9_percentile_filter} provides a glimpse of the percentile filter in action. In this case, the network is same as the one presented in Fig.~\ref{fig:3_detailed_view_sorted} and Fig.~\ref{fig:4_detailed_view_reverse_sorted} but only visualizes the filters which were most important due to the percentile filter being set to the 90\textsuperscript{th} percentile.

\begin{figure*}[!h]
    \centering
    \includegraphics[width=0.78\textwidth]{Images/9_percentile-crop1.png}
\caption{Application of the percentile filter on the detailed view (Second level)} 
    \label{fig:9_percentile_filter}
\end{figure*}

The visualization enabled a detailed inspection of the network which highlighted many different aspects of the network's learning.

\begin{itemize}
\item Most of the filters in the network were useless i.e. they contributed nothing to the final prediction for that particular input. These filters changed as the stimulus to the network changed indicating that some filters were specialized in a particular input.
\item Many of the filters had very similar activating patterns in the network which were assigned to the same filter cluster. This highlighted the aspect of lack of diversity in the trained network.
\item Despite of the improvement in performance with the addition of the first-order derivative of the original signal, most of the filters strongly attended to the original signal as compared to the first-order derivative.
\end{itemize}



